Unsupervised Representation Learning by Balanced Self Attention Matching

Many leading self-supervised methods for unsupervised representation learning, in particular those for embedding image features, are built on variants of the instance discrimination task, whose optimization is known to be prone to instabilities that can lead to feature collapse. Different techniques have been devised to circumvent this issue, including the use of negative pairs with different contrastive losses, the use of external memory banks, and breaking of symmetry by using separate encoding networks with possibly different structures. Our method, termed BAM, rather than directly matching features of different views (augmentations) of input images, is based on matching their self-attention vectors, which are the distributions of similarities to the entire set of augmented images of a batch. We obtain rich representations and avoid feature collapse by minimizing a loss that matches these distributions to their globally balanced and entropy regularized version, which is obtained through a simple self-optimal-transport computation. We ablate and verify our method through a wide set of experiments that show competitive performance with leading methods on both semi-supervised and transfer-learning benchmarks. Our implementation and pre-trained models are available at github.com/DanielShalam/BAM .

==> analysis.tex <==



==> experiments.tex <==
\vspace{-0.4em}
We assess the performance of \algo 's representation %\footnote{Our training code and pre-trained models will be publicly released at a later date.}  %\footnote{Our training code and pre-trained models will be publicly released at \url{https://github.com/deepmind/deepmind-research/tree/master/byol}.}  
after self-supervised pretraining on the training set of the ImageNet ILSVRC-2012 dataset~\cite{ILSVRC15}. We first evaluate it on ImageNet (IN) in both linear evaluation and semi-supervised setups. We then measure its transfer capabilities on other datasets and tasks, including classification, segmentation, object detection and depth estimation. For comparison, we also report scores for a representation trained using labels from the \texttt{train\xspace} ImageNet subset, referred to as \supervisedbaseline. In \Cref{app:train-places}, we assess the generality of \algo by pretraining a representation on the Places365-Standard dataset~\cite{zhou2017places} before reproducing this evaluation protocol.

\vfill
\paragraph{Linear evaluation on ImageNet}
We first evaluate \algo's representation by training a linear classifier on top of the frozen representation, following the procedure described in~\cite{kolesnikov2019revisiting,kornblith2019better,Zhang2016ColorfulIC,CPC,SimCLR}, and \cref{app:linear_eval_details}; we report top-$1$ and top-$5$ accuracies in \% on the \texttt{test\xspace} set in \Cref{table:linear_classif}. With a standard ResNet-$50$ ($\times 1$) \algo obtains $74.3\%$ top-$1$ accuracy ($91.6\%$ top-$5$ accuracy), which is a $1.3\%$ (resp.\,$0.5\%$) improvement over the previous self-supervised state of the art~\cite{Tian2020WhatMF}. This tightens the gap with respect to the supervised baseline of~\cite{SimCLR}, $76.5\%$, but is still significantly below the stronger supervised baseline of~\cite{gong2020maxup}, $78.9\%$. With deeper and wider architectures, \algo consistently outperforms the previous state of the art (\Cref{app:larger_architectures}), and obtains a best performance of $79.6\%$ top-$1$ accuracy, ranking higher than previous self-supervised approaches. On a ResNet-$50$ ($4\times$) \algo achieves $78.6\%$, similar to the $78.9\%$ of the best supervised baseline in \cite{SimCLR} for the same architecture. 

\vfill

\begin{table}[h]
\begin{subtable}{.38\linewidth}
    \small
    \centering
    \begin{tabular}[t]{l l r r r}
    \toprule
         Method &  Top-$1$ & Top-$5$ \\
         \midrule
         Local Agg.\,& $60.2$ & -\\
         \PIRL \cite{PIRL} & $63.6$ & -\\
         \CPCC \cite{CPCv2} & $63.8$ & $85.3$\\
         \CMC \cite{CMC} & $66.2$ & $87.0$\\
         \simclr \cite{SimCLR} & $69.3$ & $89.0$\\
         \moco v2 \cite{MOCOv2} & $71.1$ & -\\
         InfoMin Aug.\,\cite{Tian2020WhatMF} & $73.0$ & $91.1$\\
         \algo (ours) & $\cellcolor{pearDark!20}\bf{74.3}$ & $\cellcolor{pearDark!20}\bf{91.6}$\\
         \bottomrule
\end{tabular}
     \caption{\label{table:linear_classif_1}ResNet-50 encoder.}
\end{subtable}
\hfill
\begin{subtable}{.62\linewidth}
     \small
    \centering
    \begin{tabular}[t]{l l r r r}
    \toprule
    Method & Architecture & Param. &  Top-$1$ & Top-$5$ \\
    \midrule 
         \simclr \cite{SimCLR}      & ResNet-$50$ ($2\times$)  & $94$M  & $74.2$ & $92.0$\\
         \CMC \cite{CMC}            & ResNet-$50$ ($2\times$)  & $94$M  & $70.6$ & $89.7$\\
         \algo (ours)               & ResNet-$50$ ($2\times$)  & $94$M  & \cellcolor{pearDark!20} $77.4$ & \cellcolor{pearDark!20} $93.6$\\
         \CPCC \cite{CPCv2}         & ResNet-$161$             & $305$M & $71.5$ & $90.1$\\
         \moco \cite{MOCO}          & ResNet-$50$ ($4\times$)  & $375$M & $68.6$ & -\\
         \simclr \cite{SimCLR}      & ResNet-$50$ ($4\times$)  & $375$M & $76.5$ & $93.2$\\
         \algo (ours)               & ResNet-$50$ ($4\times$)  & $375$M & $\cellcolor{pearDark!20}78.6$ &\cellcolor{pearDark!20} $94.2$\\
         \algo (ours)               & ResNet-$200$ ($2\times$) & $250$M & $\cellcolor{pearDark!20}\bf{79.6}$ &\cellcolor{pearDark!20} $\bf{94.8}$\\
         \bottomrule
    \end{tabular}
     \caption{\label{table:linear_classif_2}Other ResNet encoder architectures.}
\end{subtable}
\caption{\label{table:linear_classif}Top-1 and top-5 accuracies (in \%) under linear evaluation on ImageNet.}
%\vspace{-1.4em}
\vspace{-0.5em}
\end{table}

\vfill
\paragraph{Semi-supervised training on ImageNet} 
Next, we evaluate the performance obtained when fine-tuning \algo's representation on a classification task with a small subset of ImageNet's \texttt{train\xspace} set, this time using label information. We follow the semi-supervised protocol of~\cite{kornblith2019better,dmlab,SimCLR,CPCv2} detailed in \Cref{app:semi_sup_details}, and use the same fixed splits of respectively $1\%$ and $10\%$ of ImageNet labeled training data as in~\cite{SimCLR}. We report both top-$1$ and top-$5$ accuracies on the  \texttt{test\xspace} set in \Cref{table:few_labels}. \algo consistently outperforms previous approaches across a wide range of architectures. 
Additionally, as detailed in \Cref{app:semi_sup_details}, \algo reaches $77.7\%$ top-$1$ accuracy with ResNet-50 when fine-tuning over $100\%$ of ImageNet labels. 

\vfill

\begin{table}[h]
\setlength\tabcolsep{3.5pt}
\begin{subtable}{.4\linewidth}
    \small
    \centering
    \begin{tabular}{l r r r r}
\toprule
    Method     & \multicolumn{2}{c}{Top-$1$} & \multicolumn{2}{c}{Top-$5$} \\
              &  $1\%$ & $10\%$            & $1\%$ & $10\%$ \\
    \midrule
    Supervised~\cite{zhai2019s4l} & $25.4$ & $56.4$ & $48.4$ & $80.4$ \\
    \midrule
    InstDisc                 & - & -                     & $39.2$ & $77.4$\\
    PIRL \cite{PIRL}         & - & -                     & $57.2$ & $83.8$\\
    \simclr \cite{SimCLR}    & $48.3$ & $65.6$           & $75.5$ & $87.8$\\
    \algo (ours)             & \cellcolor{pearDark!20} $\bf{53.2}$ & \cellcolor{pearDark!20} $\bf{68.8}$ &\cellcolor{pearDark!20} $\bf{78.4}$ & \cellcolor{pearDark!20} $\bf{89.0}$\\
    \bottomrule
\end{tabular}
\vspace{0.5em}
\caption{ResNet-50 encoder. }
\end{subtable}
\hfill
\begin{subtable}{.6\linewidth}
    \small
    \centering
    \begin{tabular}{l l r r r r r}
    \toprule
         Method     & Architecture & Param. & \multicolumn{2}{c}{Top-$1$} & \multicolumn{2}{c}{Top-$5$} \\
                    &              &         & $1\%$ & $10\%$            & $1\%$ & $10\%$ \\
         \midrule
         \CPCC \cite{CPCv2}       & ResNet-$161$            & $305$M     & - & - & $77.9$ & $91.2$\\
         \simclr \cite{SimCLR}    & ResNet-$50$ ($2\times$) & $94$M         & $58.5$ & $71.7$ & ${83.0}$ & $91.2$\\
          \algo (ours)            & ResNet-$50$ ($2\times$) & $94$M         & \cellcolor{pearDark!20} ${62.2}$ & \cellcolor{pearDark!20} ${73.5}$ &\cellcolor{pearDark!20} ${84.1}$              & \cellcolor{pearDark!20} ${91.7}$\\
         \simclr \cite{SimCLR}    & ResNet-$50$ ($4\times$) & $375$M     & $63.0$ & $74.4$ & $85.8$ & ${92.6}$\\
         \algo (ours)             & ResNet-$50$ ($4\times$) & $375$M     &\cellcolor{pearDark!20} ${69.1}$& \cellcolor{pearDark!20} ${75.7}$ &\cellcolor{pearDark!20} ${87.9}$ &\cellcolor{pearDark!20} $92.5$\\
         \algo (ours)             & ResNet-$200$ ($2\times$) & $250$M    &\cellcolor{pearDark!20} $\bf{71.2}$ & $\cellcolor{pearDark!20}\bf{77.7}$ &\cellcolor{pearDark!20} $\bf{89.5}$ &\cellcolor{pearDark!20} $\bf{93.7}$\\
         \bottomrule
    \end{tabular}
    \vspace{0.5em}
\caption{Other ResNet encoder architectures.}
\end{subtable}
% \begin{subtable}{.4\linewidth}
%     \small
%     \centering
%     \begin{tabular}{l r r r r r r}
% \toprule
%     Method     & \multicolumn{3}{c}{Top-$1$} & \multicolumn{3}{c}{Top-$5$} \\
%               &  $1\%$ & $10\%$ & $100\%$            & $1\%$ & $10\%$ & $100\%$ \\
%     \midrule
%     Supervised~\cite{zhai2019s4l} & $25.4$ & $56.4$ & $76.4$ & $48.4$ & $92.9$ \\
%     \midrule
%     %InstDisc                 & - & - & -                     & $39.2$ & $77.4$ & -\\
%     %PIRL \cite{PIRL}         & - & - & -                     & $57.2$ & $83.8$ & -\\
%     \simclr \cite{SimCLR}    & $48.3$ & $65.6$ & $76.0$          & $75.5$ & $87.8$ & $93.1$\\
%     \algo (ours)             & \cellcolor{pearDark!20} $\bf{53.2}$ & \cellcolor{pearDark!20} $\bf{68.8}$  & \cellcolor{pearDark!20} $\bm{77.7}$ &\cellcolor{pearDark!20} $\bf{78.4}$ & \cellcolor{pearDark!20} $\bf{89.0}$ & \cellcolor{pearDark!20} $\bm{93.9}$\\
%     \bottomrule
% \end{tabular}
% \vspace{0.5em}
% \caption{ResNet-50 encoder. }
% \end{subtable}
% \hfill
% \end{subtable}
% \begin{subtable}{.6\linewidth}
%     \small
%     \centering
%     \begin{tabular}{l l r r r r r}
%     \toprule
%          Method     & Architecture & Param. & \multicolumn{2}{c}{Top-$1$} & \multicolumn{2}{c}{Top-$5$} \\
%                     &              &         & $1\%$ & $10\%$            & $1\%$ & $10\%$ \\
%          \midrule
%          \CPCC \cite{CPCv2}       & ResNet-$161$            & $305$M     & - & - & $77.9$ & $91.2$ \\
%             \algo          & ResNet-$50$ ($1\times$) & $24$M         & ${62.2}$ & ${73.5}$ & ${84.1}$ &  ${91.7}$\\
%           \algo             & ResNet-$50$ ($2\times$) & $94$M         & ${62.2}$ & ${73.5}$ & ${84.1}$ &  ${91.7}$\\
%          \algo              & ResNet-$50$ ($4\times$) & $375$M     & ${69.1}$&  ${75.7}$ & ${87.9}$ & $92.5$\\
         
%          \algo              & ResNet-$200$ ($2\times$) & $250$M    & $\bf{71.2}$ & $\bf{77.7}$ & $\bf{89.5}$ & $\bf{93.7}$\\
%          \bottomrule
%     \end{tabular}
%\end{subtable}
\caption{\label{table:few_labels}Semi-supervised training with a fraction of ImageNet labels.}


%\vspace{-1.4em}
\vspace{-0.8em}
\end{table}


\paragraph{Transfer to other classification tasks} We evaluate our representation on other classification datasets to assess whether the features learned on ImageNet (IN) are generic and thus useful across image domains, or if they are ImageNet-specific.
We perform linear evaluation and fine-tuning on the same set of classification tasks used in~\cite{SimCLR,kornblith2019better}, and carefully follow their evaluation protocol, as detailed in \Cref{app:transfer_details}. Performance is reported using standard metrics for each benchmark, and results are provided on a held-out \texttt{test\xspace} set after hyperparameter selection on a validation set. We report results in \Cref{tab:transfer_learning}, both for linear evaluation and fine-tuning. \algo outperforms \simclr on all benchmarks and the \supervisedbaseline~baseline on $7$ of the $12$ benchmarks, providing only slightly worse performance on the $5$ remaining benchmarks. \algo's representation can be transferred over to small images, e.g., CIFAR~\cite{cifar}, landscapes, e.g., SUN397~\cite{sun397} or VOC2007~\cite{pascal}, and textures, e.g., DTD~\cite{dtd}.

\begin{table}[t]
    \centering
    \scriptsize
    \input{tables/transfer_table.tex}
     \vspace{0.5em}
     \caption{Transfer learning results from ImageNet (IN) with the standard ResNet-50 architecture.}
     \label{tab:transfer_learning}
     \vspace{-0.8em}
\end{table}

\paragraph{Transfer to other vision tasks} We evaluate our representation on different tasks relevant to computer vision practitioners, namely semantic segmentation, object detection and depth estimation. With this evaluation, we assess whether \algo's representation generalizes beyond classification tasks.

We first evaluate \algo on the VOC2012 semantic segmentation task as detailed in~\Cref{app:semantic_seg}, where the goal is to classify each pixel in the image~\cite{long2015fully}. We report the results in \Cref{tab:detect_segment}. \algo outperforms both the \supervisedbaseline~baseline ($+1.9$ mIoU) and \simclr ($+1.1$ mIoU).

Similarly, we evaluate on object detection by reproducing the setup in~\cite{MOCO} using a Faster R-CNN architecture~\cite{ren2015faster}, as detailed in~\Cref{app:object_det}. We fine-tune on  \texttt{trainval2007\xspace} and report results on  \texttt{test2007\xspace} using the standard AP$_{50}$ metric; \algo is significantly better than the \supervisedbaseline~baseline ($+3.1$ AP$_{50}$) and \simclr ($+2.3$ AP$_{50}$).

Finally, we evaluate on depth estimation on the NYU v2 dataset, where the depth map of a scene is estimated given a single RGB image. Depth prediction measures how well a network represents geometry, and how well that information can be localized to pixel accuracy~\cite{doersch2017multi}. The setup is based on~\cite{laina2016depth} and detailed in \Cref{app:depth}. We evaluate on the commonly used  \texttt{test\xspace} subset of $654$ images and report results using several common metrics in \Cref{table:depth}: relative (rel) error, root mean squared (rms) error, and the percent of pixels (pct) where the error, $\max (d_{gt}/d_{p}, d_{p}/d_{gt})$, is below $1.25^{n}$ thresholds where $d_p$ is the predicted depth and $d_{gt}$ is the ground truth depth~\cite{doersch2017multi}. \algo is better or on par with other methods for each metric. For instance, the challenging pct.\,$\!\,\!<\!\!1.25$ measure is respectively improved by $+3.5$ points and $+1.3$ points compared to supervised and \simclr baselines.

\vspace{0.5em}
\begin{table}[h]
%\begin{center}
\begin{subtable}{.35\linewidth}
\small
\begin{center}
\centering\hspace*{-1.cm}
\begin{tabular}{l r r }
\toprule
    Method     & AP$_{50}$ & mIoU \\
    \midrule
    \supervisedbaseline~\cite{MOCO} & $74.4$ & $74.4$  \\
    \midrule
    MoCo~\cite{MOCO}       & $74.9$ & $72.5$\\
    \simclr (repro)  & $75.2$ & $75.2$\\
    \algo (ours)   & \cellcolor{pearDark!20} $\bf{77.5}$  & \cellcolor{pearDark!20} $\bf{76.3}$\\
    \bottomrule
\end{tabular}
\caption{\label{tab:detect_segment}Transfer results in semantic\\  segmentation and object detection.}
\end{center}
\end{subtable}
\begin{subtable}{.65\linewidth}
\small
\centering
\vspace{-0.330cm} \hspace*{-0.7cm}
\begin{tabular}{l c c c c c}
\toprule
               & \multicolumn{3}{c}{Higher better} & \multicolumn{2}{c}{Lower better}\\
    {Method}&{pct.\,$\!<\!1.25$}&{pct.\,$\!<\!1.25^2$}&{pct.\,$\!<\!1.25^3$}&{rms} &{rel}\\
    \midrule
    \supervisedbaseline~\cite{laina2016depth}&$81.1$&$95.3$&$98.8$&$0.573$&$\bf{0.127}$\\
    \midrule
    \simclr (repro) &$83.3$&$96.5$&$99.1$&$0.557$&$0.134$\\
    \algo (ours) &\cellcolor{pearDark!20}$\bf{84.6}$&\cellcolor{pearDark!20}$\bf{96.7}$& \cellcolor{pearDark!20} $\bf{99.1}$&\cellcolor{pearDark!20}$\bf{0.541}$&\cellcolor{pearDark!20}$0.129$\vspace*{-0.05cm}\\
    \bottomrule
\end{tabular}
\caption{\label{table:depth}Transfer results on NYU v2 depth estimation.}
\end{subtable}
\caption{\label{tab:other_transfer}Results on transferring \algo's representation to other vision tasks.}
\vspace{-0.8em}
%\end{center}
\end{table}
%\vspace{-1em}
